The three-component defocusing nonlinear Schrodinger equation with nonzero boundary conditions

We present a rigorous theory of the inverse scattering transform (IST) for the three-component defocusing nonlinear Schrodinger (NLS) equation with initial conditions approaching constant values with the same amplitude as $x\to\pm\infty$. The theory combines and extends to a problem with non-zero boundary conditions three fundamental ideas: (i) the tensor approach used by Beals, Deift and Tomei for $n$-th order scattering problems, (ii) the triangular decompositions of the scattering matrix used by Novikov, Manakov, Pitaevski and Zakharov for the $N$-wave interaction equations, and (iii) a generalization of the cross product via the Hodge star duality, which, to the best of our knowledge, is used in the context of the IST for the first time in this work. The combination of the first two ideas allows us to rigorously obtain a fundamental set of analytic eigenfunctions. The third idea allows us to establish the symmetries of the eigenfunctions and scattering data. The results are used to characterize the discrete spectrum and to obtain exact soliton solutions, which describe generalizations of the so-called dark-bright solitons of the two-component NLS equation.

==> cited.tex <==
appendix.tex:Next, we use a result from~\cite{gantmacher} to obtain
app_part1.tex:These results are proved much in a similar way as for the two-component case, and we refer the reader to \cite{gbdkk2015} for details.
app_part2.tex:Next, we use a result from~\cite{gantmacher} to obtain
asymptotics.tex:$f_n$ and $g_n$ from Definition \ref{d:fg} using the techniques of \cite{BDT}
directproblem.tex:As in the scalar case \cite{ZS1973}, these eigenvalues have branching.
directproblem.tex:We deal with this issue as in \cite{gbdkk2015,BP2014,FT1987,PAB2006}
directproblem.tex:(see~\cite{PAB2006} for further details).
directproblem.tex:This normalization is the generalization of the one used in \cite{gbdkk2015,BP2014} for the scalar case.
directproblem.tex:As in the focusing and defocusing Manakov system with NZBC \cite{PAB2006,gbdkk2015,KBK2015}, 
directproblem.tex:to obtain two auxiliary scattering eigenfunctions \cite{gbdkk2015,PAB2006}.  
directproblem.tex:prove analogous results (see \cite{gbdkk2015} for more details).
directproblem.tex:we use a different approach that generalizes to the $N$-component case and which was studied in Ref.~\cite{PBT2011}.
directproblem.tex:In this section and the next we show how a combination of the methods of~\cite{BDT} 
directproblem.tex:and the approach of~\cite{NMPZ1984} can be used 
directproblem.tex:We begin by briefly recalling some results from \cite{PBT2011}, where 
directproblem.tex:generalizing the approach introduced in \cite{BDT} for the $N$-th order scattering operator,
directproblem.tex:First, following \cite{PBT2011} we introduce the following quantities:
directproblem.tex:where the symbol ``$\wedge$" denotes the wedge product as in~\cite{PBT2011}.
directproblem.tex:The following result was proved in~\cite{PBT2011}:
directproblem.tex:differ slightly from those in~\cite{PBT2011}.
directproblem.tex:More precisely, in \cite{PBT2011} the ordering of the eigenvalues of $\@X_\pm$ was reversed in the LHP, and
directproblem.tex:Theorem~\ref{t:tensoranalyticity} also leads to the following result~\cite{PBT2011}:
directproblem.tex:(Again, note the slight difference between what is presented here and what was presented in~\cite{PBT2011}.)
directproblem.tex:To this end, we need the following result \cite{PBT2011}:
directproblem.tex:admit smooth extensions to $\Real \setminus \{\pm q_o\}$ \cite{PBT2011}.
directproblem.tex:Comparing this result to~\cite{PBT2011}, the slight difference is now clear:
directproblem.tex:%One can repeat the the proofs from~\cite{PBT2011} exactly, provided one takes care to note the changes in
directproblem.tex:%All of this is done to extend the claims in~\cite{NMPZ1984} to the case of the defocusing VNLS equation with NZBC.
directproblem.tex:Taking the limit $\Im z\to0^\pm$ one has \cite{PBT2011}:
directproblem.tex:Namely, generalizing ideas presented in~\cite{NMPZ1984} for a first-order matrix system with ZBC, 
directproblem.tex:Hereafter, we will use the notation of~\cite{gantmacher}:
directproblem.tex:The minors of an $N \times N$ matrix $\@A$ and those of its inverse $\@B= \@A^{-1}$ are related as follows~\cite{gantmacher}:
directproblem.tex:The connection between this work and~\cite{NMPZ1984} should now be clear.
directproblem.tex:for a general $N\times N$ scattering problem with ZBC by the authors of~\cite{NMPZ1984}.
directproblem.tex:Corollary~\ref{c:invert} are the generalizations of the similar relations valid for the Manakov system~\cite{gbdkk2015,PAB2006}.
directproblem.tex:%as \cite{gbdkk2015,PAB2006}.
directproblem.tex:The results presented in this section (i) they provide a rigorous implementation of the framework of~\cite{NMPZ1984}
directproblem.tex:For comparison purposes, recall that \cite{NMPZ1984} only considers the case of compact support and uses Fredholm integral
directproblem.tex:Similarly, no such extra analyticity properties exist for the scattering problem studied in \cite{NMPZ1984}.
directproblem.tex:No such degeneracy exists for the problem studied in \cite{NMPZ1984}, and 
introduction.tex:which possess a remarkably rich mathematical structure (e.g., see \cite{AC1991,AS1981,BBEIM,FT1987,Gesztesy,NMPZ1984} and references therein).
introduction.tex:and Bose-Einstein condensation (e.g., see \cite{AS1981,InfeldRowlands,Sulem,Whitham} and references therein).
introduction.tex:in the dynamics of two miscible superfluids experiencing fast counterflow in a narrow (cigar-shaped) condensate \cite{hoefer}. 
introduction.tex:Moreover, problems with NZBC are relevant for the study of modulational instability \cite{lombardo2,naturephys,ZO2009,zhaoliu}.
introduction.tex:In turn, the IST is based on formulating the PDE as the compatibility condition of a Lax pair \cite{lax}.
introduction.tex:The IST for the focusing NLS equation with ZBC was developed in~\cite{ZS1972} 
introduction.tex:(see also Refs.~\cite{AC1991,AS1981,NMPZ1984}).
introduction.tex:The theory was then made rigorous in \cite{BealsCoifman} (see also \cite{BDT,DeiftTrubowitz}).
introduction.tex:The IST for the defocusing scalar case with NZBC was developed in~\cite{ZS1973}, and was subsequently more rigorously revisited in
introduction.tex:\cite{FT1987,prinari2013},
introduction.tex:while the focusing case with NZBC was recently done in \cite{BK2014}.
introduction.tex:The IST for the Manakov system for the focusing case with ZBC was developed in 1974 \cite{Manakov},
introduction.tex:and the theory can be extended to an arbitrary number of components in a straightforward way \cite{APT2003}.
introduction.tex:\cite{prinari2013,FT1987},
introduction.tex:and even though the case of ZBC was settled a long time ago, some questions are still outstanding in the case of NZBC (e.g., see \cite{BF2014,BP2014}).
introduction.tex:The IST for the defocusing Manakov system with NZBC was outlined in~\cite{PAB2006},
introduction.tex:making use of an idea introduced in \cite{Kaup} to solve the IVP for the three-wave interaction equations.
introduction.tex:The problem was then rigorously revisited in~\cite{gbdkk2015}, and 
introduction.tex:the focusing Manakov system with NZBC was studied in \cite{KBK2015} using similar methods.
introduction.tex:Unfortunately, the approach used in \cite{gbdkk2015,KBK2015,PAB2006} %to to circumvent the non-analyticity issues for the Manakov system 
introduction.tex:A significant step forward for this problem was recently presented in \cite{PBT2011}.
introduction.tex:There, the methods of \cite{BDT} were generalized to systems with NZBC and degenerate eigenvalues.
introduction.tex:On the other hand, several issues were left open in \cite{PBT2011}, including the explicit construction of complete sets of analytic eigenfunctions,
introduction.tex:The second idea is the use of a triangular decomposition of the scattering matrix (generalizing the ideas of \cite{NMPZ1984}
introduction.tex:%which are derived in terms of fundamental tensors using the approach to the IST presented in \cite{PBT2011} combined with the ideas of \cite{NMPZ1984};
introduction.tex:and compared to the approach presented in \cite{gbdkk2015,PAB2006}.
inverseproblem.tex:\cite{gbdkk2015}.
inverseproblem.tex:Though a methodology to solve this problem was introduced in \cite{PAB2006} and made rigorous in \cite{gbdkk2015},
inverseproblem.tex:We again compare with the results of \cite{PBT2011} as in Theorem \ref{t:gantmacher}
inverseproblem.tex:These analyticity properties were found for the Manakov system in \cite{gbdkk2015}
inverseproblem.tex:From here, the results are the same as in \cite{gbdkk2015,PAB2006}.
inverseproblem.tex:Some such solutions were presented in \cite{PRL2015}.
inverseproblem.tex:It is well known that, for the scalar NLS equation, such singularities are not allowed in the defocusing case with NZBC \cite{FT1987},
inverseproblem.tex:but are possible in the focusing case with ZBC \cite{Zhou}.
inverseproblem.tex:the long-time asymptotic behavior using the Deift-Zhou method \cite{CPAM47p199,AM137p295} 
inverseproblem.tex:(see \cite{itsustinov,vartanian1,vartanian2} for the defocusing scalar case with NZBC)
inverseproblem.tex:that the scattering problem is not self-adjoint \cite{KBK2015}.
inverseproblem.tex:was done in \cite{BFP2015,boitipempinelli} in the defocusing case and in \cite{demontis} for the focusing case.
symmetries.tex:that is uniquely defined up to a change in sign \cite{Frankel}.
symmetries.tex:star operator, where ``$\wedge$'' is the wedge product as defined in \cite{Frankel}.
symmetries.tex:Lemma~\ref{L:adjoint} is the generalization of an analogous result for the Manakov system \cite{gbdkk2015,PAB2006}.
symmetries.tex:In~\cite{PAB2006}, the analogous result was used to construct the auxiliary eigenfunctions, 
symmetries.tex:which made it necessary to use the approach of~\cite{BDT} and~\cite{PBT2011}.
vnls3c.tex:\usepackage[colorlinks=true,linkcolor=blue,citecolor=red,bookmarksnumbered=true]{hyperref}
vnls3c.tex:[GB] Are all refs cited?

